A Replication Study on Predicting Metamorphic Relations at Unit Testing Level

Metamorphic Testing (MT) addresses the test oracle problem by examining the relations between inputs and outputs of test executions. Such relations are known as Metamorphic Relations (MRs). In current practice, identifying and selecting suitable MRs is usually a challenging manual task, requiring a thorough grasp of the SUT and its application domain. Thus, Kanewala et al. proposed the Predicting Metamorphic Relations (PMR) approach to automatically suggest MRs from a list of six pre-defined MRs for testing newly developed methods. PMR is based on a classification model trained on features extracted from the control-flow graph (CFG) of 100 Java methods. In our replication study, we explore the generalizability of PMR. First, we rebuild the entire preprocessing and training pipeline and repeat the original study in a close replication to verify the reported results and establish the basis for further experiments. Second, we perform a conceptual replication to explore the reusability of the PMR model trained on CFGs from Java methods in the first step for functionally identical methods implemented in Python and C++. Finally, we retrain the model on the CFGs from the Python and C++ methods to investigate the dependence on programming language and implementation details. We were able to successfully replicate the original study achieving comparable results for the Java methods set. However, the prediction performance of the Java-based classifiers significantly decreases when applied to functionally equivalent Python and C++ methods despite using only CFG features to abstract from language details. Since the performance improved again when the classifiers were retrained on the CFGs of the methods written in Python and C++, we conclude that the PMR approach can be generalized, but only when classifiers are developed starting from code artefacts in the used programming language.

==> metrics_DS_c++.tex <==
\extrarowheight = 0.5ex
\begin{table}[!h]
	\caption{Performance comparison for models DT, SVM,and RF using DS$_{C++}$ dataset }
	\label{tbl:stage2_DS_C++_Dataset}
	\centering
	\resizebox{0.48\textwidth}{!} {
		
		\begin{tabular}{c|c|l|l|l|l|l|l}
			\toprule
			\multirow{2}{*}{\textbf{MR}} & \multirow{2}{*}{\textbf{ML model}} &\multicolumn{6}{c} {\textbf{Performance measurements}}\\
			&&\textbf{Acc$^\perp$}&\textbf{Pre$^\pm$}&\textbf{Recall}& \textbf{f-mea$^\ddagger$}&\textbf{AUC}&\textbf{BSR$^\dagger$}\\
			\midrule
			\multirow{3}{*}{ADD} 
			& DT  &	\textbf{0.727} & 0.614 & \textbf{0.725} & 0.601 & 0.685 & 0.625 \\
            & RF  &	0.693 &	0.675 &	0.714 &	\textbf{0.743} & \textbf{0.709} & \textbf{0.726} \\
            & SVM &	0.638 &	\textbf{0.713} & 0.654 & 0.722 & 0.697 & 0.626 \\

			\midrule
			\multirow{3}{*}{MUL} 
			& DT  &	0.674 &	0.566 &	0.643 &	0.594 &	0.637 &	0.649 \\
            & RF  &	0.604 & 0.700 &	0.721 &	\textbf{0.694} & \textbf{0.730} &	\textbf{0.714} \\
            & SVM &	\textbf{0.742} & \textbf{0.746} & \textbf{0.726} & 0.673 &	0.583 &	0.686 \\

			\midrule
			\multirow{3}{*}{PER} 
			& DT  &	\textbf{0.848}& \textbf{0.817} & 0.708 & \textbf{0.825} &	0.810 &	0.690 \\
            & RF  &	0.746 &	0.813 &	\textbf{0.761} & 0.708 & 0.776 & 0.808 \\
            & SVM &	0.757 &	0.816 &	0.705 & 0.816  & \textbf{0.829} & \textbf{0.828} \\

			\midrule
			\multirow{3}{*}{INC} 
			& DT  &	\textbf{0.775} & \textbf{0.772} & \textbf{0.798} &	\textbf{0.754} & 0.675 & \textbf{0.792} \\
            & RF  &	0.709 &	0.661 &	0.684 &	0.670 &	\textbf{0.736} &	0.726 \\
            & SVM &	0.707 &	0.713 &	0.694 &	0.745 &	0.697 &	0.673 \\

			\midrule
			\multirow{3}{*}{EXC} 
			& DT  &	0.709 &	0.706 &	0.664 &	0.664 &	\textbf{0.742} &	0.683 \\
            & RF  &	\textbf{0.747} &	\textbf{0.805} &	\textbf{0.755} &	\textbf{0.809} &	0.741 &	\textbf{0.775} \\
            & SVM &	0.670 &	0.689 &	0.674 &	0.633 &	0.718 &	0.653 \\

			\midrule
			\multirow{3}{*}{INV} 
			& DT  &	0.603 &	0.567 &	0.676 &	0.570 &	0.601 &	0.657 \\
            & RF  &	\textbf{0.717} & \textbf{0.607} & \textbf{0.701} & \textbf{0.591} & \textbf{0.609} & \textbf{0.732} \\
            & SVM &	0.534 &	0.589 &	0.573 &	0.587 &	0.540 &	0.557 \\

			\bottomrule
			\multicolumn{8}{l}{{$^\perp$Accuracy,  $^\pm$Precision, $^\ddagger$f-measure, $^\dagger$Balanced Success Rate}} 
	\end{tabular}}
\end{table}


==> metrics_DS_jk.tex <==
\extrarowheight = 0.25ex
\begin{table}[!ht]
	\caption{Performance comparison for models DT, RF, and SVM using DS$_{JK}$ dataset }
	\label{tbl:stage1_DSjk_Dataset}
	\centering
	\resizebox{0.48\textwidth}{!} {
		
		\begin{tabular}{c|c|l|l|l|l|l|l}
			\toprule
			\multirow{2}{*}{\textbf{MR}} & \multirow{2}{*}{\textbf{ML model}} &\multicolumn{6}{c} {\textbf{Performance measurements}}\\
			&&\textbf{Acc$^\perp$}&\textbf{Pre$^\pm$}&\textbf{Recall}& \textbf{f-mea$^\ddagger$}&\textbf{AUC}&\textbf{BSR$^\dagger$}\\
			\midrule
			\multirow{3}{*}{ADD} 
			& DT  &	\textbf{0.772} &	0.774 &	0.708 &	0.764 &	0.762 &	0.702 \\
            & RF  &	0.730 &	\textbf{0.828} &	0.710 &	\textbf{0.830} &	\textbf{0.832} &	0.657 \\
            & SVM &	0.771 &	0.780 &	\textbf{0.807} &	0.780 &	0.784 &	\textbf{0.772} \\

			\midrule
			\multirow{3}{*}{MUL} 
			& DT  &	0.689 &	0.722 & 0.679 &	0.666 &	\textbf{0.705} &	0.709 \\
            & RF  &	0.675 &	\textbf{0.749} &	0.626 &	\textbf{0.740} &	0.689 &	0.676 \\
            & SVM &	\textbf{0.713} &	0.702 &	\textbf{0.799} &	0.680 &	0.673 &	\textbf{0.742} \\

			\midrule
			\multirow{3}{*}{PER} 
			& DT  &	0.821 &	0.847 & 0.829 &	\textbf{0.878} &	\textbf{0.895} &	\textbf{0.887} \\
            & RF  &	0.863 &	0.805 &	0.839 &	0.849 &	0.863 &	\textbf{0.887} \\
            & SVM &	\textbf{0.891} &	\textbf{0.856} &	\textbf{0.869} &	0.851 &	0.869 &	0.850 \\

			\midrule
			\multirow{3}{*}{INC} 
			& DT  &	0.787 &	0.837 &	0.785 &	0.830 &	0.798 &	0.773 \\
            & RF  &	0.755 &	0.780 &	0.733 &	0.751 &	0.772 &	0.702 \\
            & SVM &	\textbf{0.790} & \textbf{0.860} &\textbf{0.802} & \textbf{0.844} & \textbf{0.810} &	\textbf{0.845} \\
            
			\midrule
			\multirow{3}{*}{EXC} 
			& DT  &	0.798 &	0.791 &	0.795 &	0.791 &	0.789 &	0.782 \\
            & RF  &	\textbf{0.812} & \textbf{0.881} &\textbf{ 0.843} &	\textbf{0.803} & \textbf{0.876} &	\textbf{0.879} \\
            & SVM &	0.744 &	0.754 &	0.748 &	0.765 &	0.747 &	0.766 \\

			\midrule
			\multirow{3}{*}{INV} 
			& DT  &	0.683 &	0.669 &	0.675 &	\textbf{0.703} &	0.659 &	0.690 \\
            & RF  &	\textbf{0.771} & \textbf{0.776} & \textbf{0.737} &	0.700 &	\textbf{0.699} &\textbf{0.790} \\
            & SVM &	0.624 &	0.629 &	0.671 &	0.665 &	0.632 &	0.615 \\

			
			\bottomrule
			\multicolumn{8}{l}{{$^\perp$Accuracy,  $^\pm$Precision, $^\ddagger$f-measure, $^\dagger$Balanced Success Rate}} 
	\end{tabular}}
\end{table}

==> metrics_DS_jv.tex <==
\extrarowheight = 0.25ex
\begin{table}[!tp]
	\caption{Performance comparison for models DT, SVM,and RF using DS$_{JV}$ dataset }
	\label{tbl:stage1_DSjv_Dataset}
	\centering
	\resizebox{0.48\textwidth}{!} {
		
		\begin{tabular}{c|c|l|l|l|l|l|l}
			\toprule
			\multirow{2}{*}{\textbf{MR}} & \multirow{2}{*}{\textbf{ML model}} &\multicolumn{6}{c} {\textbf{Performance measurements}}\\
			&&\textbf{Acc$^\perp$}&\textbf{Pre$^\pm$}&\textbf{Recall}& \textbf{f-mea$^\ddagger$}&\textbf{AUC}&\textbf{BSR$^\dagger$}\\
			\midrule
			\multirow{3}{*}{ADD} 
			& DT  &	0.774 &	\textbf{0.806} &	0.723 &	0.706 &	\textbf{0.805}&	\textbf{0.800} \\
            & RF  &	\textbf{0.839}&	0.792 &	0.688 &	0.741 & 0.797 &	0.796 \\ 
            & SVM &	0.769 &	0.782 &	\textbf{0.793}&	\textbf{0.774} &	0.776 &	0.769 \\

			\midrule
			\multirow{3}{*}{MUL} 
			& DT  &	0.696 &	0.703 &	0.674 &	0.660 &	\textbf{0.697} &	0.633 \\
            & RF  &	0.643 &	\textbf{0.745} &	\textbf{0.760}&	0.665 &	0.665 &	\textbf{0.708} \\
            & SVM &	\textbf{0.749}&	0.740 &	0.720 &	\textbf{0.704}&	0.692 &	0.677 \\

			\midrule
			\multirow{3}{*}{PER} 
			& DT  &	0.816 &	0.837 & 0.863 &	0.819 &	\textbf{0.924} & 0.835 \\
            & RF  &	0.884 &	0.872 &	0.865 &	\textbf{0.856} &	0.848 &	0.795 \\
            & SVM &	\textbf{0.903} & \textbf{0.907} & \textbf{0.878} &	0.841 &	0.840 &	\textbf{0.868} \\

			\midrule
			\multirow{3}{*}{INC} 
			& DT  &	\textbf{0.840} & \textbf{0.834} & \textbf{0.846} &	0.823 &	0.757 &	\textbf{0.835} \\
            & RF  &	0.746 &	0.782 &	0.681 &	0.742 &	0.708 &	0.691 \\
            & SVM &	0.810 &	0.803 &	0.777 &	\textbf{0.848} &	\textbf{0.851} &	0.794 \\

			\midrule
			\multirow{3}{*}{EXC} 
			& DT  &	0.755 &	0.753 &	0.744 &	0.768 & 0.731 &	0.790 \\
            & RF  &	\textbf{0.853} &	\textbf{0.803} &	\textbf{0.796} &\textbf{0.857} &	\textbf{0.825} &	\textbf{0.798 }\\
            & SVM &	0.752 &	0.734 &	0.779 &	0.747 &	0.742 &	0.776 \\

			\midrule
			\multirow{3}{*}{INV} 
			& DT  &	0.645 &	0.703 &	0.673 &	0.689 &	0.695 &	\textbf{0.719} \\
            & RF  &	\textbf{0.711} &	\textbf{0.789} &	\textbf{0.771} &	\textbf{0.785} &\textbf{	0.767} & 0.684 \\
            & SVM &	0.605 &	0.581 &	0.675 &	0.593 &	0.612 &	0.668 \\

			\bottomrule
			\multicolumn{8}{l}{{$^\perp$Accuracy,  $^\pm$Precision, $^\ddagger$f-measure, $^\dagger$Balanced Success Rate}} 
	\end{tabular}}
\end{table}


==> metrics_DS_py.tex <==
\extrarowheight = 0.5ex
\begin{table}[!h]
	\caption{Performance comparison for models DT, RF, and SVM using DS$_{PY}$ dataset }
	\label{tbl:stage2_DSpy_Dataset}
	\centering
	\resizebox{0.48\textwidth}{!} {
		
		\begin{tabular}{c|c|l|l|l|l|l|l}
			\toprule
			\multirow{2}{*}{\textbf{MR}} & \multirow{2}{*}{\textbf{ML model}} &\multicolumn{6}{c} {\textbf{Performance measurements}}\\
			&&\textbf{Acc$^\perp$}&\textbf{Pre$^\pm$}&\textbf{Recall}& \textbf{f-mea$^\ddagger$}&\textbf{AUC}&\textbf{BSR$^\dagger$}\\
			\midrule
			\multirow{3}{*}{ADD} 
			& DT  & 0.723 &	0.679 &	0.670 &	0.730 &	0.743 &	0.689 \\
            & RF  &	0.659 &	0.729 &	0.759 &	0.613 &	\textbf{0.768} & \textbf{0.802} \\
            & SVM &	\textbf{0.737} & \textbf{0.770} & \textbf{0.747} &	\textbf{0.751} &	0.751 &	0.704 \\ 

			\midrule
			\multirow{3}{*}{MUL} 
			& DT  &	0.651 &	0.669 &	0.642 &	0.626 &	0.666 &	0.609 \\
            & RF  &	\textbf{0.734} & 0.683 & 0.628 & 0.648 &	0.609 &	0.617 \\
            & SVM &	0.708 &	\textbf{0.778} & \textbf{0.798} & \textbf{0.706} &	\textbf{0.791} & \textbf{0.747 }\\

			\midrule
			\multirow{3}{*}{PER} 
			& DT  &	0.787 &	0.852 &	\textbf{0.846}&	0.802 &	0.820 &	0.780 \\
            & RF  &	\textbf{0.833} &	0.756 &	0.778 &	0.811 &	0.780 &	\textbf{0.839} \\
            & SVM &	0.825 &	\textbf{0.858} & 0.817 & \textbf{0.830} &	\textbf{0.827} &	0.834 \\

			\midrule
			\multirow{3}{*}{INC} 
			& DT  &	0.731 &	0.755 &	\textbf{0.786} & \textbf{0.780} & \textbf{0.796} &	0.776 \\
            & RF  &	0.708 &	0.677 &	0.722 &	0.727 &	0.730 &	0.692 \\
            & SVM &	\textbf{0.743} &	\textbf{0.788} & 0.737 &	0.793 &	0.801 &	\textbf{0.787 }\\

			\midrule
			\multirow{3}{*}{EXC} 
			& DT  &	0.737 &	0.714 &	0.724 &	0.762 &	0.727 &	0.725 \\
            & RF  &	\textbf{0.750} & \textbf{0.804} & \textbf{0.789} & \textbf{0.793} &\textbf{	0.810} &	\textbf{0.814} \\
            & SVM &	0.699 &	0.726 &	0.698 &	0.724 &	0.691 &	0.724 \\

			\midrule
			\multirow{3}{*}{INV} 
			& DT  &	0.678 &	0.660 & 0.605 &	0.603 &	0.654 &	0.669 \\
            & RF  &	\textbf{0.732} & \textbf{0.718} & \textbf{0.641} &	\textbf{0.675} & \textbf{0.727} & \textbf{0.702} \\
            & SVM &	0.588 &	0.574 &	0.591 &	0.582 &	0.582 &	0.621 \\
            
			\bottomrule
			\multicolumn{8}{l}{{$^\perp$Accuracy,  $^\pm$Precision, $^\ddagger$f-measure, $^\dagger$Balanced Success Rate}} 
	\end{tabular}}
\end{table}

